Computer-Aided Data Mining: Automating a Novel Knowledge Discovery and Data Mining Process Model for Metabolomics

This work presents MeKDDaM-SAGA, computer-aided automation software for implementing a novel knowledge discovery and data mining process model that was designed for performing justifiable, traceable and reproducible metabolomics data analysis. The process model focuses on achieving metabolomics analytical objectives and on considering the nature of its involved data. MeKDDaM-SAGA was successfully used for guiding the process model execution in a number of metabolomics applications. It satisfies the requirements of the proposed process model design and execution. The software realises the process model layout, structure and flow and it enables its execution externally using various data mining and machine learning tools or internally using a number of embedded facilities that were built for performing a number of automated activities such as data preprocessing, data exploration, data acclimatization, modelling, evaluation and visualization. MeKDDaM-SAGA was developed using object-oriented software engineering methodology and was constructed in Java. It consists of 241 design classes that were designed to implement 27 use-cases. The software uses an XML database to guarantee portability and uses a GUI interface to ensure its user-friendliness. It implements an internal embedded version control system that is used to realise and manage the process flow, feedback and iterations and to enable undoing and redoing the execution of the process phases, activities, and the internal tasks within its phases.

==> figures/himet_c45_model_visualisation.tex <==
\begin{landscape}
\pagestyle {plain}
\scriptsize
%--------------------------------------------------------------------------------------------
%ffffffffffffffffffffffffffffffffffffffffffffffffffff
%\figuremacroW{HiMet_C45_model_visualisation}
%      {Visualisation of the C4.5 model in the \emph{Arabedopesis Isoprenoids Application}}
%      {An illustration of the C4.5 decision tree model}
%      {1.5}
%ffffffffffffffffffffffffffffffffffffffffffffffffffff

%ffffffffffffffffffffffffffffffffffffffffffffffffffffffffffffffffffffffff
\begin{figure}[tb!h]
\centerline{\includegraphics[width=1.45\textwidth]{figures/HiMet_C45_model_visualisation.png}}
\centering
\caption{\textbf{Visualisation of the C4.5 model in the \emph{Arabedopesis Isoprenoids Application}:} An illustration of the C4.5 decision tree model
\label{fig:HiMet_C45_model_visualisation}}
\end{figure}
%ffffffffffffffffffffffffffffffffffffffffffffffffffffffffffffffffffffffff



%--------------------------------------------------------------------------------------------
\end{landscape}

